Deep Efficient Private Neighbor Generation for Subgraph Federated Learning

Behemoth graphs are often fragmented and separately stored by multiple data owners as distributed subgraphs in many realistic applications. Without harming data privacy, it is natural to consider the subgraph federated learning (subgraph FL) scenario, where each local client holds a subgraph of the entire global graph, to obtain globally generalized graph mining models. To overcome the unique challenge of incomplete information propagation on local subgraphs due to missing cross-subgraph neighbors, previous works resort to the augmentation of local neighborhoods through the joint FL of missing neighbor generators and GNNs. Yet their technical designs have profound limitations regarding the utility, efficiency, and privacy goals of FL. In this work, we propose FedDEP to comprehensively tackle these challenges in subgraph FL. FedDEP consists of a series of novel technical designs: (1) Deep neighbor generation through leveraging the GNN embeddings of potential missing neighbors; (2) Efficient pseudo-FL for neighbor generation through embedding prototyping; and (3) Privacy protection through noise-less edge-local-differential-privacy. We analyze the correctness and efficiency of FedDEP, and provide theoretical guarantees on its privacy. Empirical results on four real-world datasets justify the clear benefits of proposed techniques.

==> 02-related.tex <==
\section{Related Works}
\label{sec:related}
\subsection{Federated Learning for Graphs}
\label{subsec:rw_fl}
With massive graph data separately stored by distributed data owners, recent research has emerged in the field of FL over graph data. Some studies propose FL methods for tasks on distributed knowledge graphs, such as recommendation or representation learning~\cite{peng2021differentially, chen2021fede, zhang2022efficient, gu2023dynamic}. Another direction is for the scenarios where every client holds a set of small graphs, such as molecular graphs for drug discovery~\cite{xie2021federated}. 
In this work, we consider subgraph FL, where each client holds a subgraph of the entire global graph, and the only central server is dataless. The instrumental isolation of data samples leads to incomplete structural features of local nodes due to cross-subgraph neighbors missing not at random, which is fundamentally different from the centralized graph learning scenarios with unbiased sparse links \cite{liu2022local} or randomized DropEdge \cite{rong2019dropedge}. 

To deal with the missing neighbor problem in subgraph FL, existing works~\cite{zhang2021subgraph,zhang2022subgraph,wu2022federated,chen2021fedgraph, pan2023lumos, zhao2022fedgsl} propose to augment local subgraphs by retrieving missing neighbors across clients, and then mend the subgraphs with the retrieved neighbor information. FedGraph~\cite{chen2021fedgraph} considers a relaxed scenario where the existences of inter-subgraph neighbors are known for corresponding clients. \red{Moreover, similar to Lumos~\cite{pan2023lumos}, it requests the central server to manage the FL process with auxiliary data.} FedSage~\cite{zhang2021subgraph} primarily focuses on the design of the missing neighbor generator without considering the important aspects of efficiency and privacy. FedHG~\cite{zhang2022subgraph} studies the heterogeneous subgraph FL systems where graphs consist of multiple types of nodes and links, and it only protects the partial privacy of certain types of nodes in the system. FedGNN~\cite{wu2022federated} \red{and FedGSL~\cite{zhao2022fedgsl} equips their augmentation with privacy protection based on %. However, compared to the system we consider, 
additional trusted authorities and/or noise injection.} % is required by FedGNN to achieve its protection. 

None of them provides a complete solution to the utility, efficiency, and privacy of subgraph FL. %All these works are deficient in efficiency as their augmentations induce substantial overhead in computation and communication. 

%Our proposed subgraph FL framework is built for subgraph FL systems and comprehensively tackles three key challenges in subgraph FL, \ie, utility, efficiency, and privacy.
\subsection{Privacy-Preserving Learning for Graphs}
\label{subsec:rw_dp}
Privacy-preserving learning over graph data has been widely studied. Differential Privacy (DP)~\cite{dwork2006differential} is a widely applied privacy concept in this field, which describes the privacy of a method in protecting individual samples while preserving the analytical properties of the entire dataset.
A prevalent approach in attaining a graph mining model with general DP is DPSGD~\cite{abadi2016deep}, which injects designed noise into clipped gradients during model training. For centralized training scenarios, DPGGAN~\cite{yang2021secure} incorporates DPSGD to achieve DP for individual links on original graphs.
In FL systems, VFGNN~\cite{zhou2021vertically} and FedGNN~\cite{wu2022federated} leverage DPSGD and cryptology techniques to obtain rigorous privacy guarantees for federated graph learning. Meanwhile, to achieve general DP on graphs, there are some other noised-injecting based methods. Previous works of centralized learning ~\cite{lu2014exponential,ahmed2019publishing,xiao2014differentially},, FKGE~\cite{peng2021differentially} \red{and FedGSL~\cite{zhao2022fedgsl}} for FL systems, guarantee their proposed techniques with general DP by applying noise perturbation. 
 %In FL systems, FKGE~\cite{peng2021differentially} is a DP framework for learning embedding from distributed knowledge graphs. Specifically, FKGE perturbs the outputs of distributed models to achieve general DP.
 %However, VFGNN studies the vertical FL system, where each client holds a fraction of features for their nodes. Though FedGNN focuses on distributed subgraphs, homomorphic encryption can result in significant additional cost for the FL system. 
 
%However, applying noise that perturbs gradients or/and outputs can significantly degenerate the final model performance.
However, general DP does not depict the protections for sensitive node features, edges, or neighborhoods, on distributed graphs. %Yet VFGNN and FedGNN only analyzes its general differential privacy for the entire system, without showing the protection for sensitive neighborhood structures of nodes in a distributed graph.
Edge local DP and node local DP (edge-LDP and node-LDP) are two specific types of DP targeting local nodes' neighbor lists~\cite{qin2017generating}. These novel DP definitions better fit the graph learning that learns from multiple neighbor lists, and match the privacy goal of protecting nodes' local neighborhoods. 

As illustrated in Definition 2.2 in~\cite{qin2017generating}, edge-LDP defines how much a model tells for two neighborhoods that differ by one edge, while node-LDP promises a model's max leakage for all possible neighborhoods. In contrast to node-LDP, which is much stronger and can severely hinder the graph model's utility, edge-LDP precisely illustrates the local DP for local neighborhoods without overly constraining the model.

% \vspace{-4pt}
% \begin{definition} [Edge Local Differential Privacy \cite{qin2017generating,liu2022collecting}]
% \label{def:edge-ldp}
% For a graph with $n$ nodes, denote its node $v$’s neighbor list as $(b_1,\dots,b_n)$. For $u\in[n]$, if $v$ is linked with \red{$u$}, $b_u$ is 1. Otherwise, $b_u$ is 0.
% Let $\varepsilon, \delta \in \mathbb{R}_{\geq 0}$, and $R: \mathcal{G} \rightarrow \mathbb{R}$ is a randomized algorithm. $R$ provides $(\varepsilon,\delta)$-edge-LDP if for any two local neighbor lists $\gamma, \gamma'$ that differ in one bit and any $S \subseteq R$,
% \vspace{-1mm}
% \begin{equation*}
% \small
%     Pr[R(\gamma) \in S] \leq e^{\varepsilon} Pr[R(\gamma') \in S]+\delta.
% \end{equation*}
% \end{definition}
% \vspace{-2mm}

There are several works analyzing edge-LDP over distributed graph data. Qin et al.~\cite{qin2017generating} propose a decentralized social graphs generation technique with the edge-LDP. Imola et al.~\cite{imola2022differentially} analyze the edge-LDP of the proposed shuffle techniques in handling the triangle and 4-cycle counting for neighbor lists of distributed users. Lin et al.~\cite{lin2022towards} propose Solitude, an edge-LDP collaborative training framework for distributed graphs, where each client shares its perturbed local graph for the training. However, different from our subgraph FL setting, its central server (data curator) has access to node identities and labels. To the best of our knowledge, we are the first to leverage edge-LDP in the FL setting.

